The Structure of Isoperimetric Bubbles on $\mathbb{R}^n$ and $\mathbb{S}^n$

The multi-bubble isoperimetric conjecture in $n$-dimensional Euclidean and spherical spaces from the 1990's asserts that standard bubbles uniquely minimize total perimeter among all $q-1$ bubbles enclosing prescribed volume, for any $q \leq n+2$. The double-bubble conjecture on $\mathbb{R}^3$ was confirmed in 2000 by Hutchings-Morgan-Ritor\'e-Ros, and is nowadays fully resolved for all $n \geq 2$. The double-bubble conjecture on $\mathbb{S}^2$ and triple-bubble conjecture on $\mathbb{R}^2$ have also been resolved, but all other cases are in general open. We confirm the conjecture on $\mathbb{R}^n$ and on $\mathbb{S}^n$ for all $q \leq \min(5,n+1)$, namely: the double-bubble conjectures for $n \geq 2$, the triple-bubble conjectures for $n \geq 3$ and the quadruple-bubble conjectures for $n \geq 4$. In fact, we show that for all $q \leq n+1$, a minimizing cluster necessarily has spherical interfaces, and after stereographic projection to $\mathbb{S}^n$, its cells are obtained as the Voronoi cells of $q$ affine-functions, or equivalently, as the intersection with $\mathbb{S}^n$ of convex polyhedra in $\mathbb{R}^{n+1}$. Moreover, the cells (including the unbounded one) are necessarily connected and intersect a common hyperplane of symmetry, resolving a conjecture of Heppes. We also show for all $q \leq n+1$ that a minimizer with non-empty interfaces between all pairs of cells is necessarily a standard bubble. The proof makes crucial use of considering $\mathbb{R}^n$ and $\mathbb{S}^n$ in tandem and of M\"obius geometry and conformal Killing fields; it does not rely on establishing a PDI for the isoperimetric profile as in the Gaussian setting, which seems out of reach in the present one.

==> cluster-stereographic-color-lightened.tex <==
\path[draw=black,join=round,line cap=round,fill=white]
(-0.17473456106980606, 0.15261593264972131)
arc (422.17767179614356:657.8223282038565:0.17256453883459194)
arc (237.8223282038588:256.90989283616875:0.18031166690864125)
arc (196.9098928361688:272.67724808823687:0.6038018934107716)
arc (212.6772480882369:507.3227519117631:1.1171254135997817)
arc (447.32275191176313:523.0901071638312:0.6038018934107716)
arc (463.09010716383125:482.17767179614117:0.18031166690864125)
;
\path[draw=black,join=round,line cap=round,fill=green!30!white]
(0.778251208361622, -0.18901250493923663)
arc (265.66191852057625:454.33808147942375:0.1895555666872178)
arc (394.33808147942403:434.2040028896514:0.3350840027383518)
arc (374.20400288965146:387.3227519117631:1.3140298727408297)
arc (507.3227519117631:212.6772480882369:1.1171254135997817)
arc (332.6772480882369:345.7959971103484:1.3140298727408297)
arc (285.79599711034854:325.66191852057597:0.3350840027383518)
;
\path[draw=black,join=round,line cap=round,fill=magenta!90!cyan!30!white]
(0.4966377525794205, 0.18552582028004236)
arc (455.6392076859911:624.3607923140089:0.1864280592536302)
arc (204.360792314009:225.79599711034854:0.4497801185622753)
arc (345.7959971103485:332.6772480882369:1.3140298727408297)
arc (272.67724808823687:196.90989283616878:0.6038018934107716)
arc (316.90989283616886:403.09010716383114:0.2570839161572535)
arc (163.09010716383125:87.3227519117631:0.6038018934107716)
arc (27.32275191176309:14.204002889651491:1.3140298727408297)
arc (494.2040028896514:515.639207685991:0.4497801185622753)
;
\path[draw=black,join=round,line cap=round,fill=red!30!white]
(-0.1747345610698039, -0.1526159326497203)
arc (357.8223282038565:362.1776717961435:4.016378630787581)
arc (122.1776717961412:103.09010716383122:0.18031166690864125)
arc (403.09010716383114:316.90989283616886:0.2570839161572535)
arc (256.90989283616875:237.8223282038588:0.18031166690864125)
;
\path[draw=black,join=round,line cap=round,fill=yellow!30!white]
(-0.1747345610698039, -0.15261593264972081)
arc (357.8223282038565:362.1776717961435:4.016378630787581)
arc (62.177671796143564:297.82232820385644:0.17256453883459194)
;
\path[draw=black,join=round,line cap=round,fill=blue!30!white]
(0.7782512083616212, 0.18901250493923666)
arc (514.3380814794239:565.6619185205761:0.43645791675086554)
arc (325.66191852057597:285.79599711034854:0.3350840027383518)
arc (225.79599711034854:204.360792314009:0.4497801185622753)
arc (324.36079231400913:395.63920768599087:0.31840128691061304)
arc (155.639207685991:134.20400288965146:0.4497801185622753)
arc (74.20400288965143:34.338081479424005:0.3350840027383518)
;
\path[draw=black,join=round,line cap=round,fill=violet!30!white]
(0.4966377525794208, -0.18552582028004194)
arc (324.3607923140091:395.6392076859909:0.31840128691061304)
arc (95.6392076859911:264.3607923140089:0.1864280592536302)
;
\path[draw=black,join=round,line cap=round,fill=orange!30!white]
(0.7782512083616212, 0.1890125049392366)
arc (154.33808147942386:205.66191852057614:0.43645791675086554)
arc (265.66191852057625:454.33808147942375:0.1895555666872178)
;

